Simplified Models for Dark Matter Searches at the LHC

This document outlines a set of simplified models for dark matter and its interactions with Standard Model particles. It is intended to summarize the main characteristics that these simplified models have when applied to dark matter searches at the LHC, and to provide a number of useful expressions for reference. The list of models includes both s-channel and t-channel scenarios. For s-channel, spin-0 and spin-1 mediation is discussed, and also realizations where the Higgs particle provides a portal between the dark and visible sectors. The guiding principles underpinning the proposed simplified models are spelled out, and some suggestions for implementation are presented.

==> Makefile <==
LATEX    = pdflatex
BIBTEX   = bibtex
DVIPS    = dvips

BASENAME = dmlhc2014

default: testpdflatex

testlatex:
	latex  ${BASENAME}
	latex  ${BASENAME}
	bibtex ${BASENAME}
	latex  ${BASENAME}
	latex  ${BASENAME}
	dvipdf -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress ${BASENAME}

testpdflatex:
	pdflatex  ${BASENAME}
	pdflatex  ${BASENAME}
#       bibtex    ${BASENAME}
	pdflatex  ${BASENAME}
	pdflatex  ${BASENAME}

#
# standard Latex targets
#

%.dvi:  %.tex 
	$(LATEX) $<

%.bbl:  %.tex *.bib
	$(LATEX) $*
	$(BIBTEX) $*

%.ps:   %.dvi
	$(DVIPS) $< -o $@

%.pdf:  %.tex
	$(PDFLATEX) $<

.PHONY: clean

clean:
	rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg  \
	      *.inx *.dvi *.toc *.out *~ ~* spellTmp 

